HUP-3D: A 3D multi-view synthetic dataset for assisted-egocentric hand-ultrasound pose estimation

We present HUP-3D, a 3D multi-view multi-modal synthetic dataset for hand-ultrasound (US) probe pose estimation in the context of obstetric ultrasound. Egocentric markerless 3D joint pose estimation has potential applications in mixed reality based medical education. The ability to understand hand and probe movements programmatically opens the door to tailored guidance and mentoring applications. Our dataset consists of over 31k sets of RGB, depth and segmentation mask frames, including pose related ground truth data, with a strong emphasis on image diversity and complexity. Adopting a camera viewpoint-based sphere concept allows us to capture a variety of views and generate multiple hand grasp poses using a pre-trained network. Additionally, our approach includes a software-based image rendering concept, enhancing diversity with various hand and arm textures, lighting conditions, and background images. Furthermore, we validated our proposed dataset with state-of-the-art learning models and we obtained the lowest hand-object keypoint errors. The dataset and other details are provided with the supplementary material. The source code of our grasp generation and rendering pipeline will be made publicly available.

==> bibliography_backup.tex <==
\bibitem{Hasson2020Leveraging}
Yana Hasson, Bugra Tekin, Federica Bogo, Ivan Laptev, Marc Pollefeys, and Cordelia Schmid.
\newblock Leveraging Photometric Consistency Over Time for Sparsely Supervised Hand-Object Reconstruction.
\newblock In \textit{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, June 2020.


\bibitem{jiang2021graspTTA}
H. Jiang, S. Liu, J. Wang, and X. Wang, ``Hand-Object Contact Consistency Reasoning for Human Grasps Generation,'' in \textit{Proceedings of the International Conference on Computer Vision}, 2021.

\bibitem{Akin2012Enhanced}
Abdulkadir Akin, E. Erdede, Hossein Afshari, Alexandre Schmid, and Yusuf Leblebici.
\newblock Enhanced Omnidirectional Image Reconstruction Algorithm and Its Real-Time Hardware.
\newblock In \textit{Proceedings - 15th Euromicro Conference on Digital System Design, DSD 2012}, pages 907--914. September 2012.
\newblock \doi{10.1109/DSD.2012.52}.
\newblock ISBN 978-1-4673-2498-4.

\bibitem{Liu2021SemiSupervised}
Shaowei Liu, Hanwen Jiang, Jiarui Xu, Sifei Liu, and Xiaolong Wang.
\newblock Semi-Supervised 3D Hand-Object Poses Estimation With Interactions in Time.
\newblock In \textit{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, pages 14687--14697, June 2021.

\bibitem{Oberweger2020Generalized}
Markus Oberweger, Paul Wohlhart, and Vincent Lepetit.
\newblock Generalized Feedback Loop for Joint Hand-Object Pose Estimation.
\newblock \textit{IEEE Transactions on Pattern Analysis and Machine Intelligence}, 42(8):1898--1912, 2020.
\newblock \doi{10.1109/TPAMI.2019.2907951}.

% Dataset papers ------------------------------------
\bibitem{hasson19_obman}
Y. Hasson, G. Varol, D. Tzionas, I. Kalevatykh, M. J. Black, I. Laptev, and C. Schmid, "Learning joint reconstruction of hands and manipulated objects," in \textit{Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}, 2019.

\bibitem{Hein2021}
Hein, J., Seibold, M., Bogo, F., Farshad, M., Pollefeys, M., Fürnstahl, P. and Navab, N. (2021). Towards markerless surgical tool and hand pose estimation. International Journal of Computer Assisted Radiology and Surgery, 16(5), 799–808. https://doi.org/10.1007/s11548-021-02369-2

\bibitem{wang2023pov}
R. Wang, S. Ktistakis, S. Zhang, M. Meboldt, and Q. Lohmeyer, "POV-Surgery: A Dataset for Egocentric Hand and Tool Pose Estimation During Surgical Activities," in \textit{Proceedings of the International Conference on Medical Image Computing and Computer-Assisted Intervention}, 2023, pp. 440--450.

\bibitem{GRAB:2020}
O. Taheri, N. Ghorbani, M. J. Black, and D. Tzionas, ``{GRAB}: A Dataset of Whole-Body Human Grasping of Objects,'' in \textit{Proceedings of the European Conference on Computer Vision (ECCV)}, 2020. [Online]. Available: \url{https://grab.is.tue.mpg.de}

\bibitem{Hampali2020HOnnotate}
Shreyas Hampali, Mahdi Rad, Markus Oberweger, and Vincent Lepetit.
\newblock HOnnotate: A Method for 3D Annotation of Hand and Object Poses.
\newblock In \textit{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, June 2020.

\bibitem{Brahmbhatt2020ContactPose}
Samarth Brahmbhatt, Chengcheng Tang, Christopher D. Twigg, Charles C. Kemp, and James Hays.
\newblock ContactPose: A Dataset of Grasps with Object Contact and Hand Pose.
\newblock In Andrea Vedaldi, Horst Bischof, Thomas Brox, and Jan-Michael Frahm, editors, \textit{Computer Vision -- ECCV 2020}, pages 361--378. Springer International Publishing, Cham, 2020.
\newblock ISBN 978-3-030-58601-0.

\bibitem{Doosti2020HOPENet}
Bardia Doosti, Shujon Naha, Majid Mirbagheri, and David J. Crandall.
\newblock HOPE-Net: A Graph-Based Model for Hand-Object Pose Estimation.
\newblock In \textit{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, June 2020.

\bibitem{kwon2021h2o}
T. Kwon, B. Tekin, J. Stühmer, F. Bogo, and M. Pollefeys, ``H2O: Two hands manipulating objects for first person interaction recognition,'' in \emph{Proceedings of the IEEE/CVF International Conference on Computer Vision}, pp. 10138--10148, 2021.

\bibitem{moon2020interhand2}
G. Moon, S.-I. Yu, H. Wen, T. Shiratori, and K. M. Lee, ``Interhand2.6m: A dataset and baseline for 3d interacting hand pose estimation from a single RGB image,'' in \emph{Computer Vision--ECCV 2020: 16th European Conference, Glasgow, UK, August 23--28, 2020, Proceedings, Part XX 16}, pp. 548--564, Springer, 2020.

\bibitem{garcia2018first}
G. Garcia-Hernando, S. Yuan, S. Baek, and T.-K. Kim, ``First-person hand action benchmark with RGB-D videos and 3D hand pose annotations,'' in \emph{Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition}, pp. 409--419, 2018.

%---------------------------------------------------

\bibitem{miller2004graspit}
Andrew T. Miller and Peter K. Allen.
\newblock Graspit! A Versatile Simulator for Robotic Grasping.
\newblock \textit{IEEE Robotics \& Automation Magazine}, 11(4):110--122, 2004.
\newblock IEEE.

\bibitem{Blender2018}
Blender Online Community.
\newblock \textit{Blender - a 3D modelling and rendering package}.
\newblock Stichting Blender Foundation, Amsterdam, 2018.
\newblock Available at \url{http://www.blender.org}.

\bibitem{Romero2017EmbodiedHands}
Javier Romero, Dimitrios Tzionas, and Michael J. Black.
\newblock Embodied hands: modeling and capturing hands and bodies together.
\newblock \textit{ACM Transactions on Graphics}, 36(6):245, November 2017.
\newblock Association for Computing Machinery, New York, NY, USA.
\newblock ISSN 0730-0301.
\newblock \doi{10.1145/3130800.3130883}.
\newblock Available at \url{https://doi.org/10.1145/3130800.3130883}.

\bibitem{Dromey2020DimensionlessUltrasound}
B. P. Dromey, S. Ahmed, F. Vasconcelos, E. Mazomenos, Y. Kunpalin, S. Ourselin, J. Deprest, A. L. David, D. Stoyanov, and D. M. Peebles, ``Dimensionless squared jerk: An objective differential to assess experienced and novice probe movement in obstetric ultrasound,'' \emph{Prenatal Diagnosis}, vol. 11, pp. pd.5855, 2020. [Online]. Available: https://onlinelibrary.wiley.com/doi/10.1002/pd.5855. DOI: 10.1002/pd.5855

\bibitem{CAI2020101762}
Y. Cai, R. Droste, H. Sharma, P. Chatelain, L. Drukker, A. T. Papageorghiou, and J. A. Noble, ``Spatio-temporal visual attention modelling of standard biometry plane-finding navigation,'' \emph{Medical Image Analysis}, vol. 65, pp. 101762, 2020. [Online]. Available: https://www.sciencedirect.com/science/article/pii/S1361841520301262. DOI: https://doi.org/10.1016/j.media.2020.101762

\bibitem{prokudin2019efficient}
Sergey Prokudin, Christoph Lassner, and Javier Romero.
\newblock Efficient learning on point clouds with basis point sets.
\newblock In \emph{Proceedings of the IEEE/CVF International Conference on Computer Vision}, pages 4332--4341, 2019.

\bibitem{varol2017learning}
G. Varol, J. Romero, X. Martin, N. Mahmood, M.J. Black, I. Laptev, and C. Schmid.
\newblock Learning from synthetic humans.
\newblock In: \emph{Proceedings of the IEEE conference on computer vision and pattern recognition}, pages 109--117, 2017.

\bibitem{stirnemann2020intergrowth}
Stirnemann J, Salomon LJ, Papageorghiou A.
\textit{INTERGROWTH-21st standards for Hadlock's estimation of fetal weight}.
Ultrasound Obstet Gynecol. 2020;56(6):946--948.

% Markerless surgical hand tracking from video
\bibitem{azari2019using}
D. P. Azari, Y. H. Hu, B. L. Miller, B. V. Le, and R. G. Radwin, ``Using surgeon hand motions to predict surgical maneuvers,'' \emph{Human Factors}, vol. 61, no. 8, pp. 1326--1339, 2019, SAGE Publications Sage CA: Los Angeles, CA.


% NON-image based External hand motion analysis (sensor based motion behavior) in other clinical tasks
\bibitem{8610321}
X.-H. Zhou, G.-B. Bian, X.-L. Xie, Z.-G. Hou, X. Qu, and S. Guan, ``Analysis of Interventionalists’ Natural Behaviors for Recognizing Motion Patterns of Endovascular Tools During Percutaneous Coronary Interventions,'' \emph{IEEE Transactions on Biomedical Circuits and Systems}, vol. 13, no. 2, pp. 330-342, 2019. DOI: 10.1109/TBCAS.2019.2892411.

% Motion behavior in obstetrics ultrasound
\bibitem{droste2020automatic}
R. Droste, L. Drukker, A. T. Papageorghiou, and J. A. Noble, ``Automatic probe movement guidance for freehand obstetric ultrasound,'' in \emph{Medical Image Computing and Computer Assisted Intervention--MICCAI 2020: 23rd International Conference, Lima, Peru, October 4--8, 2020, Proceedings, Part III 23}, pp. 583--592, Springer, 2020.

% Surgical skill assessment
\bibitem{goodman2021real}
E. D. Goodman, K. K. Patel, Y. Zhang, W. Locke, C. J. Kennedy, R. Mehrotra, S. Ren, M. Y. Guan, M. Downing, H. W. Chen, et al., ``A real-time spatiotemporal AI model analyzes skill in open surgical videos,'' \emph{arXiv preprint arXiv:2112.07219}, 2021.


% Surgical TOOLS-based skill assessment (laparoscopic videos)
% tracking and analyzing tool movements in surgical video
\bibitem{Jin2018ToolDetection}
A. Jin et al., ``Tool Detection and Operative Skill Assessment in Surgical Videos Using Region-Based Convolutional Neural Networks,'' in \emph{2018 IEEE Winter Conference on Applications of Computer Vision (WACV)}, Lake Tahoe, NV, USA, 2018, pp. 691-699. DOI: 10.1109/WACV.2018.00081.
\bibitem{papp2022surgical}
D. Papp, R. Nagyné Elek, and T. Haidegger, ``Surgical tool segmentation on the jigsaws dataset for autonomous image-based skill assessment,'' in \emph{2022 IEEE 10th Jubilee International Conference on Computational Cybernetics and Cyber-Medical Systems (ICCC)}, pp. 000049--000056, IEEE, 2022.

% Surgical skill assessment based on videos in robotic surgery
\bibitem{lajko2021endoscopic}
G. Lajkó, R. Nagyné Elek, and T. Haidegger, ``Endoscopic image-based skill assessment in robot-assisted minimally invasive surgery,'' \emph{Sensors}, vol. 21, no. 16, p. 5412, 2021, MDPI.
\bibitem{law2017surgeon}
H. Law, K. Ghani, and J. Deng, ``Surgeon technical skill assessment using computer vision based analysis,'' in \emph{Machine Learning for Healthcare Conference}, pp. 88--99, PMLR, 2017.

% Mixed reality: marker-based probe tracking for ultrasound-guided procedures
\bibitem{nguyen2022holous}
T. Nguyen, W. Plishker, A. Matisoff, K. Sharma, and R. Shekhar, ``HoloUS: Augmented reality visualization of live ultrasound images using HoloLens for ultrasound-guided procedures,'' \emph{International Journal of Computer Assisted Radiology and Surgery}, vol. 17, no. 2, pp. 385--391, 2022, Springer.

\bibitem{MANO:SIGGRAPHASIA:2017}
J. Romero, D. Tzionas, and M. J. Black, ``Embodied Hands: Modeling and Capturing Hands and Bodies Together,'' \emph{ACM Transactions on Graphics, (Proc. SIGGRAPH Asia)}, vol. 36, no. 6, 245:1--245:17, Nov. 2017.


\bibitem{hope}
B. Doosti, S. Naha, M. Mirbagheri and D. Crandall, ``HOPE-Net: A Graph-based Model for Hand-Object Pose Estimation'', The IEEE Conference on Computer Vision and Pattern Recognition (CVPR), June, 2020.

\bibitem{graphunet}
H. Gao and S. Ji, ``Graph U-Nets", ICML, 2019 


==> sections/obsolete_method.tex <==
\section{Method}
\begin{figure}
\includegraphics[width=\textwidth]{Figures/grasp_rendering_pipeline.pdf}
%\caption{Grasp generation and rendering pipeline overview: Grasp samples from pre-trained CoarseNet and RefineNet model %sequences are fed into a Blender-based grasp rendering concept that uses a camera view angle sphere concept to generate grasp %view angles covering a larger image variety. After adding hand and arm texture, lighting and a background image, the rendered %RGB, Depth, RGB+ground truth and segmentation images, as separate ground truth data files are being generated per image.} 
\vspace*{-6mm}
\caption{\small \textbf{Grasp generation and rendering pipeline overview:} (Upper part, grasp generation): A MANO right hand model with initial pose $[\gamma, \theta_{wrist}]$ and Basis Point Set (BPS)-encoded~\cite{prokudin2019efficient} point cloud representations of the Voluson model $\Omega_{Vert}$ whose orientation is defined by a hardcoded list of Euler angles $\Theta_{Vol}$ are fed into CoarseNet that samples full hand poses $[\gamma^{*}, \theta_{full\_pose}]$ from a 16 dimensional normal distributed latent space. The subsequent RefineNet uses computed 3D vertex deltas between the sampled hand and Voluson model $\Omega_{Vert}$ to sample refined hand poses $[\gamma^{**}, \theta^{*}_{full\_pose}]$ with optimized positional hand-probe differences. CoarseNet and RefineNet are taken from~\cite{wang2023pov}. (Lower part, grasp rendering): Blender rendering concept: The final hand pose $[\gamma^{**}, \theta^{*}_{full\_pose}]$ from the grasp generation sequence is fed into our Blender rendering concept, together with Voluson and MANO right hand model vertices $\Omega_{Vert}$ and $M_{Vert}$ and a SMPL-H body model. Within the Blender rendering sequence the generated probe poses $\gamma_{\omega}$ are z-offset-corrected via $\gamma^{\Delta}_{\omega} = \gamma_{\omega} + (0, 0, \Delta z |~\Delta z = -0.072)$ in order to account for the CoarseNet-related z-direction offset of the probe. Camera viewpoint Euler rotation angles $\Theta_{k}$ are generated from our sphere concept which creates N viewpoints using an egocentric sphere radius. We hide all SMPHL-H body parts except the right hand and arm, add hand glove and arm texture in addition to a defined set of 8 background images and random righting, and render RGB-D, segmentation map and annotation frames.}
\label{fig:pipeline_overview}
\end{figure}

%TODO refer to force-closure concept of Graspit! and mention that it was too difficult to manually generate force-closure grasps using the Voluson (easier to gef FC grasps with a surgical drill as seen in Hein et al.)

%Also mentioned that Hein et al. published synthetic and real image datasets. \newline

%TODO HONNOTATE - We were not able to install HOnnotate. Therefore we could not annotate real images and focus in synthetic images only.

%We focused on the generation of synthetic images in obstetric ultrasound scanning scenarios.
Focusing on potential medical education applications in the context of obstetric ultrasound, our joint 3D hand-probe pose estimation framework is tailored to images that show a hand holding an ultrasound probe in a clinical setup. 
Our concept can be split into three categories: grasp generation, grasp rendering and pose estimation, which will be described in detail in the following subsections. An overview of the pipeline is depicted in Fig. \ref{fig:pipeline_overview}. 


\subsection{Grasp generation}
For the sake of simplicity when it comes to ground truth annotation, we focused on a purely synthetic grasp image generation concept and didn't attempt to setup and annotate real images. An interesting option for markerless annotation of real images seemed to be the HOnnotate method~\cite{Hampali2020HOnnotate} which automatically annotates hand and object poses in each frame from recorded RGB-D camera sequences, but our attempts to install one of its dependencies, the DIRT differentiable renderer\footnote{\url{https://github.com/pmh47/dirt}}, were unsuccessful. Nevertheless, we may still explore this option in the near future. 
The underlying idea in pursuing a purely synthetic image generation approach is to explore the possibility of generating a sufficiently large variety of training images that allow acceptable generalizability to real images in pose prediction.
Our grasp generation concept focuses on a 3D scanned model of a Voluson\texttrademark~E10 probe \footnote{\url{https://www.gehealthcare.com/products/ultrasound/voluson}} since Voluson ultrasound scanners are widely used in obstetrics.

\subsubsection{Discarded Graspit! tool considerations}
\textcolor{red}{[[TODO move this to supplementary material]]}
The initial core idea of generating grasps was inspired by~\cite{hasson19_obman} and~\cite{Hein2021}, namely using the robotic grasping simulator software Graspit!~\cite{miller2004graspit}, which requires a model of robotic hand or gripper and an object model to be grasped by the robot. Instead of a robotic end effector, the methods presented in~\cite{hasson19_obman} and~\cite{Hein2021} used a MANO hand model~\cite{Romero2017EmbodiedHands} along with tangible graspable object models. 
Graspit! offers a principal component analysis (PCA) based concept called ``Eigengrasp'' to reduce complexity when representing robotic hand or gripper postures which leads to a restricted joint angle configuration space when using the MANO hand model. Considering that Graspit! is designed for robot models with potentially smaller hand posture configuration space, the use of the MANO human hand model has limitations in generating a greater variety of plausible hand grasps.  

The simulator offers configurable optimization algorithm based automated grasp finding algorithms that are based on a concept called ``Eigengrasp planning'' and were used in~\cite{hasson19_obman} for grasping every day objects from various hand angles. Such an automated grasp finding approach had to be replaced by a manual grasp template generation in~\cite{Hein2021} due to the additional constraint of hand grasps following certain orientations when holding a surgical drill. 

Initially, we followed the manual grasp template generation approach mentioned above using the Voluson probe model, which had to be discarded due to several constraints: Firstly,~\cite{Hein2021} considered grasp templates to be valid if they fulfilled Graspit!'s form-closure criterion\footnote{\url{https://graspit-simulator.github.io/build/html/gfo.html}}. The combination of MANO hand model and Voluson proved to be rather disadvantageous when it came to finding plausible form-closure grasps. Secondly, even finding plausible manual, non-optimization algorithm based grasps after deactivating the form-closure criterion turned out to be difficult due to the restricted user options when performing the ``auto grasp'' option that led to very unnatural grasps.

\subsubsection{A GrabNet derivative - Using a pre-trained generative model for joint 3D hand-object pose estimation}
\label{sec:grasp_generation}
Due to the initial limitations in generating plausible grasps with Graspit!, we used another method named POV-Surgery~\cite{wang2023pov} that is based on  GrabNet~\cite{GRAB:2020}, a generative model for joint 3D grasp pose estimation. GrabNet consists of two sequential models, CoarseNet and RefineNet, and is trained for the MANO right hand model only using every day objects such as binoculars, mugs and cameras. POV-Surgery applied GrabNet's pose prediction training and evaluation capabilities in a surgical context using surgical tools. Using multi-camera body motion capture, plausible temporal image sequences were rendered to depict surgical activities.
In our attempt, to simplify the conceptualization of a reliable data generation pipeline, we did not rely on a body motion capturing sequence, and focused on a single image generation concept instead.

Using POV-Surgery's grasp generation sequence with a defined set of Euler rotation angles for the probe mesh, denotated as $\Theta_{Vol}:= \left\{ \left[\alpha_i, \beta_i, \gamma_i\right] \right\}_{i=1}^{n} \subseteq \mathbb{R}^{3}$ \textcolor{red}{[TODO: @Razvan: replace n with  the real number of hardcoded Euler angles from which the final 11 grasps were selected, add the list of Euler angles to the table and refer to the table here]}, instead of randomly generated Euler angles, we created 11 plausible grasps via pre-trained GrabNet-based CoarseNet and SparseNet models. 
$\Theta_{Vol}$ is used to create Basis Point Set (BPS)-encoded~\cite{prokudin2019efficient} point cloud representations of the Voluson model, which serve as an input to GrabNet's encoder, together with the MANO right hand model's initial translation and orientation vectors, $\gamma \in \mathbb{R}^{3}$ respectively and $\theta_{wrist}$. CoarseNet was pre-trained on other everyday objects but conditions on the Voluson's object shape and samples from a normal distributed latent space that contains encoded 16 dimensional grasp data $Z \in \mathbb{R}^{16}$. The decoder generates a full hand pose $[\gamma^{*}, \theta_{full\_pose}]$. 
%(hand translation $\gamma^{*}$ and full hand pose incl. hand orientation and finger joint orientations $\theta_{full\_pose}$).
 CoarseNet's initial grasps are then further refined in RefineNet which takes the initial hand pose $[\gamma^{*}, \theta_{full\_pose}]$ as input, together with the Voluson model's vertices $\Omega_{Vert}$ and the distances between the hand and object vertices $\Delta^{hand}_{obj}$. The refined hand pose, denoted as $\Psi := [\gamma^{**}, \theta^{*}_{full\_pose}]$, serves as the basis for our grasp rendering concept, described in section \ref{section:grasp_rendering}.

\begin{figure}[ht]
\centering
% First subfigure with TikZ for label placement
\begin{subfigure}[b]{0.2\textwidth}
   \centering
   \begin{tikzpicture}
       \node[inner sep=0pt] (image1) {\includegraphics[width=\textwidth]{Figures/grasp_comparison.pdf}};
       \draw[orange,thick] (image1.south west) rectangle (image1.north east);
       % Label (a) positioned at the lower left corner within the bounding box
       \node[anchor=south west, fill=white, opacity=0.5, text opacity=1, inner sep=2pt] at (image1.south west) {(a)};
   \end{tikzpicture}
   %\caption{}
   \label{fig:grasp_comparison}
\end{subfigure}
%\hfill % Optionally add space between the subfigures if needed
% Second subfigure with adjusted label (b)
\begin{subfigure}[b]{0.79\textwidth}
        \centering
        \begin{tikzpicture}
            \node[inner sep=0pt] (image2) {\includegraphics[width=\textwidth]{Figures/camera_sphere_concept_diagram_final.pdf}};
            \draw[orange,thick] (image2.south west) rectangle (image2.north east);
            % Label (b) positioned at the lower left corner within the bounding box
            \node[anchor=south west, fill=white, opacity=0.5, text opacity=1, inner sep=2pt] at (image2.south west) {(b)};
        \end{tikzpicture}
        %\caption{}
        \label{fig:camera_sphere_details_diagram}
\end{subfigure}
\vspace*{-10mm}
\caption{\small (a) Illustration of grasp conversion from GrabNet, visualized via MeshLab (above) to our Blender concept (below) using an additional probe z-axis offset correction $\Delta z$. (b) Schematic camera view related details of the grasp rendering pipeline: (1) Blender scene with SMPL-H body model holding the Voluson probe and schematic egocentric camera, which we extend to non-egocentric camera views as well. (2) Right arm of SMPL-H body model after the remaining parts have been hidden and schematic camera orientations around the arm giving an impression of the camera sphere concept. (3)  Visualized camera view angle sphere concept with sample images from different latitude floors (hand mesh in the sphere center; Sphere radius and surface circle radius denoted as $r_{sphr}$ and $r_{circ}$). (4) Schematic Blender camera view of a single sphere-based camera orientation illustrating the final rendered hand and probe without added light source and background.}
\label{fig:grasp_comparison_and_camera_sphere_details_diagram}
\end{figure}


\footnotetext{\url{https://www.meshlab.net/}}

\subsection{Grasp rendering}
\label{section:grasp_rendering}
Following the general idea of a Blender-based grasp rendering concept of~\cite{Hein2021}, we adjusted our rendering pipeline in order to accept the GrabNet and RefineNet-based generated grasps $\Psi$, described in section \ref{sec:grasp_generation}. Details of the grasp rendering part can be found in the lower part of Fig.~\ref{fig:pipeline_overview}.
The current grasp generation implementation of~\cite{wang2023pov} on which our concept is based, creates .mat files which contain all grasp relevant information, and are converted into .json files in the rendering module. While our applied Blender concept places the Voluson at its origin, the converted hand grasp pose $\Psi$ expects the probe model to have a displacement on the positive z-axis of a fixed magnitude $\Delta z = 0.07189549170510294$.
We calculated $\Delta z$ programmatically by computing the translation offset between the Voluson model $\gamma^{**}$ located at its origin and the respective model which is used in the GrabNet-based grasp generation concept. 
We then applied the probe's translation offset and invert the direction of the z-axis in order to account for Blender's coordinate system representation. The Blender-internal probe location in the global coordinate system, denoted as $\gamma_{\omega}$, gets z-offset corrected as follows:
\begin{equation}
    \gamma^{\Delta}_{\omega} = \gamma_{\omega} + (0, 0, \Delta z) 
\end{equation}
Fig.~\ref{fig:grasp_comparison_and_camera_sphere_details_diagram}a schematically illustrates the probe's z-offset correction.

The Blender rendering concept also requires a SMPL-H body model, a MANO right hand model ($M_{Vert}$) and vertices of the Voluson probe model ($\Omega_{Vert}$).

We replaced the camera view Euler angles concept of~\cite{Hein2021}, which focused on purely egocentric views sampled with random variations, with a sphere concept described in section \ref{sec:sphere_concept} and illustrated in Fig.~\ref{fig:pipeline_overview} and Fig.~\ref{fig:grasp_comparison_and_camera_sphere_details_diagram}b. For each grasp generated by the grasp generation module one synthetic image per camera view angle $\Theta_k \in \left\{\Theta_1, ..., \Theta_N\right\}$ is created, where $N$ is the total number of camera views along the sphere's surface.
%We set the sphere's radius, which corresponds a plausible head-hand distance, to $r = 0.8$, because we found that %the resulting 

For each synthesized Blender image a pre-defined hand and arm texture color is being applied (out of 2 glove colors and 1 arm skin color), as well as a random background image out of a defined set of 8 images, in addition to a random light source constellation.
The final output of the rendering model is a set of images including RGB, Depth, Depth (hand only), Depth (probe only), RGB, RGB (without probe), RGB (without hand), RGB with ground truth visualization, segmentation map and ground truth data. 

\subsubsection{Camera view angle sphere concept}
\label{sec:sphere_concept}
 Instead of rendering hand-probe grasp poses from random egocentric camera angles, we use a defined set of camera angles that follow a sphere surface concept similar to~\cite{Akin2012Enhanced}, and combine egocentric with non-egocentric grasp images in order to increase the image variety. The sphere concept is defined as follows:
 %\subsubsection{Spherical Coordinates System}
Every 3D point $P$ in spherical coordinates $(r_{sph}, \theta, \phi)$ is related to Cartesian coordinates $(x, y, z)$ as follows:
\begin{equation}
x = r_{sph} \sin(\theta) \cos(\phi), \quad y = r_{sph} \sin(\theta) \sin(\phi), \quad z = r_{sph} \cos(\theta) \label{eq:1}
\end{equation}
where:
$r_{sph}$ is the radius from the origin to $P$,
$\theta$ is the polar angle of the positive $z$-axis (0 to $\pi$),
$\phi$ is the azimuthal angle of the positive $x$-axis in the $x$-$y$ plane (0 to $2\pi$).

%\subsubsection{Camera Locations Distribution}
The distribution of camera locations across a sphere is described by evenly spacing points along the latitude ($\theta$) and longitude ($\phi$) lines.

%\subsubsection{Latitude Floors}

The sphere is divided into horizontal floors based on the latitude angle $\theta$. Each latitude floor represents a different value of $\theta$. Defining $r_{circ}$ as the radius of the surface circles around each camera location, the number of floors is determined by:
\begin{equation}
N_{\text{latitude\_floors}} = \left[ \frac{\pi}{2 \arcsin\left(\frac{r_{circ}}{r_{sph}}\right)} \right]
\end{equation}


For each latitude floor $i$, the number of circles (with the camera being located in the circle centre) that can fit on the sphere's surface is given by:
\begin{equation}
N_{\text{circles}}^{(i)} = \left[ \frac{2 \pi r_{sph} \sin(\theta_i)}{2r_{circ}} \right]
\end{equation}

For each latitude floor $i$ and each surface circle $j$ on that floor, the spherical coordinates of a camera location are defined as:
\begin{equation}
(\theta_i, \phi_j^{(i)}) \quad \text{where} \quad \phi_j^{(i)} = j \cdot \Delta\phi^{(i)}, \quad j = 0, 1, \dots, N_{\text{circles}}^{(i)} - 1
\end{equation}
\vspace{-5mm}
 \begin{equation}
\Delta\phi^{(i)} = \frac{2\pi}{N_{\text{circles}}^{(i)}} N_{\text{circles}}^{(i)} - 1
\end{equation}
We included additional camera location coordinates at the 'north pole' and 'south pole' of the sphere as follows: 
North pole ($\theta = 0$): $(x = 0$, $y = 0$, $z = r)$ and south pole ($\theta = \pi$): $(x = 0$, $y = 0$, $z = -r)$.

The Euler angles $\Theta_k \in \left\{\Theta_1, ..., \Theta_N\right\} $ can be calculated from the Cartesian coordinates as follows:
\begin{align}
\text{$\Theta_{roll}$} &= \arctan2(y, x),\quad \text{$\Theta_{pitch}$} = \arctan2(-z, \sqrt{x^2 + y^2}) \\
%\text{$\Theta_{pitch}$} &= \arctan2(-z, \sqrt{x^2 + y^2}) \\
\text{$\Theta_{yaw}$} &= -\arctan2(\sin(\Theta_{roll}) \cdot z, \cos(\Theta_{roll}) \cdot x - \sin(\Theta_{roll}) \cdot y)
\end{align}
To convert these Euler angles to degrees and ensure they are within the range \([0, 360]\), the following conversions are applied:
\begin{equation}
\text{$(\Theta_\text{<axis>})$}_\text{deg} = (\Theta_\text{<axis>} \times \frac{180}{\pi}) \,\%\, 360,\, \quad \text{<axis>} \in [roll, pitch, yaw]\\
%\text{$(\Theta_{pitch})$}_\text{deg} &= (\Theta_{pitch} \times %\frac{180}{\pi}) \,\%\, 360 \\
%\text{$(\Theta_{yaw})$}_\text{deg} &= (\Theta_{yaw} \times \frac{180}%{\pi}) \,\%\, 360
\end{equation}

 Fig. \ref{fig:grasp_comparison_and_camera_sphere_details_diagram}b shows our python visualization that we used to define useful camera locations placed along the sphere's surface and pointing towards the centre, at which we placed a right hand mesh for visual inspection of the camera location's plausibility. 
The sphere is defined by its radius and the radius of the circles located around each camera location. Each circle is located adjacent to all of its neighbours with a minimum of circle overlap.
Applied in the context of the Blender scene, the distance between the camera and the right hand denotes the sphere's radius.
%In the Blender scene the camera is located at the SMPL-H body model's head and points towards the right hand.
Camera view angles that show non-plausible content such as the inside of the SMPL-H body model's arm were manually excluded.
For each generated grasp one image per camera sphere view angle was generated. 

\subsubsection{Blender-based frame rendering}
In order to favor a high variability of the rendered grasp images, several parameters can be defined that also influence the total number of rendered images (Table \ref{tab:frame_generation_config}):

\begin{table}
\caption{Frame generation configuration \textcolor{red}{TODO: add the Euler angles list that generated the final 11 grasps}}\label{tab:frame_generation_config}
\scriptsize
\begin{tabular}{l m{4.8cm} m{5.5cm}}
\hline
\textbf{Variable} & \textbf{Description} & \textbf{Values} \\ \hline
$(\Theta_{Vol})_{j}$ & k-th ($k \in [1, .., N]$) probe rotation Euler angles & \textcolor{red}{[330, 0, 0] x 10 --> TODO: @Razvan: replace $N$ by actual nr or Euler angles you've used to generate all grasps, and add these Euler angles}  \\
$(G_{[\Theta_{Vol}]})_k$ & k-th manually selected GrabNet-based grasp out of all grasps generated by $\Theta_{Vol}$ & 11 manually selected plausible grasps via visual inspection in MeshLab\\
$r_{sph}$ & Sphere radius &  0.8m \\ 
$r_{circ}$ & Sphere surface circle radius & 0.15m \\
$\Theta_k$ & k-th ($k \in [1, .., 92]$) camera view point Euler angles that depend on $r_{sph}$ and $r_{circ}$ & 92 - 2 excluded = 90 values. Concrete Euler angles can be derived from applying the sphere concept described in section \ref{sec:sphere_concept} \\ 
$z_{ego}$ & Camera distance (egocentric \newline head to hand distance) & $[0.5, 0.8]$ \\
$\mathcal{G}_{bkgr}$ & Background image for rendered \newline grasp frames & 1 x plain white, 1 x consultation room, 3 x SPACE-FAN phantom, 3 x real pregnant mother belly (white / brown / black)\\
$H_{rgb}$ & RGB values of glove texture & 
$[0.5647058824, 0.5921568627, 0.768627451]$, $[0.38039215686, 0.61960784314, 0.8666666667]$
%\vspace{-5mm}
%\[
%\left( \begin{array}{c}
%\!0.5647058824\! \\
%\!0.5921568627\! \\
%\!0.768627451\! \\
%\end{array} \right),
%\left(\begin{array}{c}
%\!0.38039215686\! \\
%\!0.61960784314\! \\
%\!0.8666666667\! \\
%\end{array}\right)
%\] \\ 
\\
$A_{rgb}$ & RGB values of the arm &
%\vspace{-5mm}
%\[
%\left(\begin{array}{c}
%\!1.0\! \\
%\!0.6784313725\! \\
%\!0.3764705882\! \\
%\end{array}\right)
%\] 
%\vspace{-2mm}\\
$[1.0, 0.6784313725, 0.3764705882]$ \\
\hline
\end{tabular}
\end{table}

We use two blue glove colors, one skin color, random scene lightning and a set of 8 background images including a laboratory setup with a SPACE-FAN ultrasound examination fetus\footnote{\url{https://www.kyotokagaku.com/en/products\_data/us-7\_en/}}, a consultation room, a plain white background and real mother's bellies. Since our focus lies on joint 3D hand-tool pose estimation, the arm texture only serves as an additional visual cue and therefore we found that using one skin color only is sufficient. \textcolor{red}{[[TODO: Maybe justify the use of only one arm skin color in a better way]]} 
Using the variable notations of table~\ref{tab:frame_generation_config}, the combinatorics for frame generation in our dataset can be expressed as follows:
%\begin{equation}
%total_{\text{grasps}} = \Theta \; \times \; rot_{x, y, z} \; \times \; z_{\text{dist}} \; \times \; glove_{\text{rgb}} \; \times \; %grasp_{<\text{bkgr}>}
%\end{equation}
\vspace{-5mm}
{
\begin{algorithm}
\scriptsize
\caption{Combinatorics for generation of frames $F$ based on a selected grasp $(G_{[\Theta_{Vol}]})_k$}
\begin{algorithmic}[1]
\Statex \hspace{-5mm} $F \gets \{Generate((G_{[\Theta_{Vol}]})_k, z_{ego}, \mathcal{G}_{bkgr}, H_{rgb}, \Theta_k, r_{sph}, r_{circ}) \,|\, \forall (G_{[\Theta_{Vol}]})_k, z_{ego}, \mathcal{G}_{bkgr}, H_{rgb}, \Theta_k\}$
\end{algorithmic}
\end{algorithm}

}


\subsubsection{Dataset comparison}
\label{sec:dataset_comparison}

%\caption{Comparison of Hand Grasp Datasets. Acronyms: $F_{No}$: Number of %frames; $I_{Src}$: Image source (R: Real, S: Synthetic, H: Hybrid); %$C_{c}$: Clinical context (yes (+)/no(-)); $L_{GT}$: Ground Truth Label %(S: Synthetic, M: Manual, H: Hardware sensors, NN: Neural network), %$M_{\neg}$: Markerless?; $Obj_{No}$: Number of objects; %$Cam^{\Theta}_{No}$: Number of camera views; $H^R_{L}$: Used hands %(Left(L), Right(R), Both(B)); $Gr_{No}$: Number of grasps; %$Cam^{\Delta}_{No}$: Number of camera distances; $Mod$: Image modality}

\begin{table}[ht]
\caption{\small \textbf{Comparison of Hand Grasp Datasets}. \small Acronyms per column: 
['\textbf{\# frames'}: S = Synthetic, R= Real]; 
['\textbf{Image source}': R = Real, S = Synthetic]; 
['\textbf{Labelling}': Syn. = Synthetic]; 
['\textbf{Used hands}': L = Left hand, R = Right hand, B = Both hands];
['\textbf{Camera view concept}': $\Theta$ = Euler angle rotation values]; 
['\textbf{Image modality}': All = RGB + Depth + Segmentation (without contact poses), All-D: RGB + Segmentation, but without Depth, RGB-D+C = RGB-D + Object contact pose ]}
\label{tab:hand_grasp_datasets}
\centering
\tiny % Makes the text size smaller
\begin{tabular}%{p{1.7cm}|p{0.8cm}|p{0.5cm}|p{0.4cm}|p{0.6cm}|p{0.5cm}|p{0.8cm}|p{0.5cm}|p{0.8cm}|p{0.5cm}|p{0.6cm}|p{0.5cm}|p{0.5cm}|p{0.9cm}|p{0.7cm}}
%{c p{0.8cm}ccp{1.0cm}ccp{1.5cm}cp{1.0cm}p{1.5cm}p{1.0cm}}
{l@{\hspace{5pt}} p{0.8cm}@{\hspace{5pt}} l@{\hspace{5pt}} l@{\hspace{5pt}} p{1.0cm}@{\hspace{5pt}} l@{\hspace{5pt}} l@{\hspace{5pt}} p{1.5cm}@{\hspace{5pt}} l@{\hspace{5pt}} p{1.0cm}@{\hspace{5pt}} p{1.4cm}@{\hspace{5pt}} p{0.5cm}}

\hline
\textbf{Dataset} & 
\centering \rotatebox[origin=c]{90}{\textbf{\#~frames}}  & 
\centering \rotatebox[origin=c]{90}{\textbf{Image source}} & 
\centering \rotatebox[origin=c]{90}{\textbf{Clinical?}} & 
\centering \rotatebox[origin=c]{90}{\parbox{1.5cm}{\textbf{Labeling}}} & 
\centering \rotatebox[origin=c]{90}{\parbox{1.5cm}{\textbf{Markerless?}}} &  
\centering \rotatebox[origin=c]{90}{\textbf{\#~clinical tools}} &  
\centering \rotatebox[origin=c]{90}{\parbox{1.5cm}{\textbf{Camera view concept}}} & 
\centering \rotatebox[origin=c]{90}{\parbox{1.5cm}{\textbf{Used hands}}} & 
\centering \rotatebox[origin=c]{90}{\parbox{1.5cm}{\textbf{\#~grasps}}} & 
\centering \rotatebox[origin=c]{90}{\parbox{1.5cm}{\textbf{\#~camera distances}}} & 
 \rotatebox[origin=c]{90}{\parbox{1.5cm}{\centering \textbf{Image modality}}}  \\ \hline
% Example row, replace "xxx" with actual data
ObMan~\cite{hasson19_obman} & 153K & S & $-$  & Syn. & \checkmark  & 0%2.7K  
& $\Theta \sim (SO(3))$ & R & 21K & Z$\sim$[0.5, 0.8] & All\\ 

HO-3D~\cite{Hampali2020HOnnotate} & 77558 & R & $-$  & NNetw. & \checkmark & 0%10 
& unknown & R & multi-view recordings & 77558 & RGB  \\

Hein et al.~\cite{Hein2021} & 10500S/ 3746R & R+S & \checkmark  & Syn./3D p.-cloud & \checkmark & 1 & egocentric sampling& R & 7$+$random variation & Z$\sim$[0.3, 0.5] & All  \\ 

POV-Surgery~\cite{wang2023pov} & 88329 & S & \checkmark & Syn. & \checkmark & 3 & egocentric body movement sequences & R & 30 key poses/ sequence & unknown & All  \\ 

ContactPose~\cite{Brahmbhatt2020ContactPose} & >2.9M & R & x & Thermal cam., Mocab, keypoint detector & $-$ & 0 & multi-view recordings & B & >2.9M & unknown & RGB-D+C \\ 

\textbf{HUP-3D (ours)} & 31680 & S & \checkmark & Syn. & \checkmark & 1 & egocentric head hand distance $+$ camera view sphere & R & 11 & $[0.5, 0.8]$ & All  \\ 
%Example & xxx & R/S & \checkmark $-$ & ... & $+$, $-$ & & ... & $\square$ %& \checkmark & ... & ... & ...  & RGB+D \\ 
\hline
\end{tabular}
\end{table}



\subsection{Joint 3D hand-probe pose estimation}

==> sections/related_works.tex <==
\subsection{Related work}

%Several works have been presented within the last five years that focus on marker-less joint hand-object pose estimation, since %markers come with the inherent risk of pose prediction bias. 

In general, joint 3D hand-object pose prediction methods can be categorized into single-frame and multi-frame concepts. In terms of generating image datasets with respective accurate 3D joint hand-pose annotations for network training, broadly two categories can be distinguished: real images and synthetic images. Ground truth annotation may be easier in synthetic image generation pipelines if 3D models of hand and object are used in 3D modelling software such as Blender~\cite{Blender2018}, such synthetic data often carries the risk of showing too little pose and/or background variety. On the other hand, when solely relying on real images for training joint 3D hand-pose prediction networks, ground truth annotation can be challenging due to the additional requirement of pose measuring hardware such as optical or inertial markers. Such markers are present in the captured images which increases the risk of pose prediction bias. 

\subsubsection{Single-frame joint hand-tool pose estimation methods}
Pioneering work on 3D hand-object pose estimation based on an end-to-end model was presented in~\cite{hasson19_obman}, that leveraged the MANO hand model~\cite{Romero2017EmbodiedHands} and a robotic grasping tool~\cite{miller2004graspit} for grasp pose generation. Grasp rendering was realized using the Blender 3D modelling software using rendering scenes comprised of the MANO hand mapped onto the the SMPL-H body model~\cite{Romero2017EmbodiedHands}. 

A follow up work~\cite{Hein2021} builds on the concept of~\cite{hasson19_obman}, but restricts the rendered synthetic Blender images to surgical egocentric scenarios in which a surgical drill is required. Since a surgical drill constraints hand poses in terms of the tool's contact surface areas and relative hand orientation, the use of Graspit! regarding grasp posture generation was limited to manual grasps unlike the Graspit!-based automated optimization algorithm used in in~\cite{hasson19_obman}. 

 In~\cite{Hampali2020HOnnotate} a MANO hand model based 3D annotation method of real images is proposed which supports a multi-camera and a single-camera setup: In the single-camera setup grasp pose estimation is realized via a temporal frame sequence, while in the multi-camera setup a combination of initial single-frame hand-object pose estimation, followed by a multi-frame pose refinement step.  
 
\subsubsection{Multi-frame joint hand-tool pose estimation methods}
A method that addresses a common constraint of real datasets being only sparely manually annotated with joint 3D hand-object poses is presented in~\cite{Hasson2020Leveraging}. The underlying assumption of this work, which uses RGB video frame sequences, is that temporal constraints exist between adjacent frames in a video sequence which can be used to predict unlabeled frames.
In~\cite{Liu2021SemiSupervised} a semi-supervised learning concept is presented that uses an initial model trained on a fully human annotated dataset which is evaluated on a video dataset to generate pseudo labels. These pseudo labels are selected leveraging spatial-temporal consistency across video frames and fed into the initial model for self-training.

\subsubsection{Hand-object datasets}
Hand-tool grasp image datasets fall into synthetic and real categories. Synthetic images, created with 3D rendering software and based on 3D hand and object models, have built-in ground truth but may lack the detail and diversity needed for models to generalize well. Real images capture authentic scenarios similar to unseen data conditions but require manual ground truth annotation through external hardware like wearable sensors or multi-camera setups.

Hasson et al.\cite{hasson19_obman} presented a dataset of synthetic everyday hand-object interactions, leveraging a robotic grasping simulator software\cite{miller2004graspit} to automatically generate plausible grasps through software-internal optimization algorithms. 
Hein et al.~\cite{Hein2021} build on the concept of Hasson et al. on, but focused on mixed reality based egocentric concept, using a surgical drill and its inherent restrictions in terms of grasp-related plausible hand orientations and contact regions. Therefore, grasping simulator-based manual grasp templates were randomly augmented to generate grasp variety.  

to egocentric camera viewpoints and released a dataset of synthetic and real surgical drill grasp images, annotated with stereo-calibrated Azure Kinect DK cameras.

Addressing the restrictions of the dataset presented in~\cite{Hein2021} of being 1.) less diverse and 2.) single-image based and thereby ignoring temporal information in surgical activities,~\cite{wang2023pov} proposed another synthetic dataset, which is based on motion capture to generate realistic body motion sequences during surgical activities while focusing on three orthopedic surgical tools: scalpel, friem and diskplacer.  

Using an automated Convolutional Neural Network (CNN)-based 3D hand-object pose annotation method that requires prior RGB-D camera recordings of hand manipulation sequences, the authors of~\cite{Hampali2020HOnnotate} generated the first dataset of real images with markerless 3D hand-object pose annotations. 

